LooPy: A Research-Friendly Mix Framework for Music Information Retrieval on Electronic Dance Music

Music information retrieval (MIR) has gone through an explosive development with the advancement of deep learning in recent years. However, music genres like electronic dance music (EDM) has always been relatively less investigated compared to others. Considering its wide range of applications, we present a Python package for automated EDM audio generation as an infrastructure for MIR for EDM songs, to mitigate the difficulty of acquiring labelled data. It is a convenient tool that could be easily concatenated to the end of many symbolic music generation pipelines. Inside this package, we provide a framework to build professional-level templates that could render a well-produced track from specified melody and chords, or produce massive tracks given only a specific key by our probabilistic symbolic melody generator. Experiments show that our mixes could achieve the same quality of the original reference songs produced by world-famous artists, with respect to both subjective and objective criteria. Our code is accessible in this repository: https://github.com/Gariscat/loopy and the official site of the project is also online https://loopy4edm.com .

==> old.tex <==
\begin{comment}
    In this subsection, we introduce the way we construct the template for several EDM genres. We currently focus on progressive house music featuring styles of several best-known leading artists in the industry, including \cite{MG, Tobu, Dubvision}, etc. The reason why we selected these artists is that they are leading the mainstream progressive house music from festivals to radios. In other words, most progressive house tracks feature one of these styles. We expect to cover most tracks using these arrangement styles, so that our generated data show close resemblance to existing popular house music.
    
    An example of style parameters is shown in Listing 1. We pre-define the names of lead layers, chord layers, bass layers and sub-bass layers and fix the volume of different channels.
    
    \lstset{basicstyle=\footnotesize, backgroundcolor=\color{white}, captionpos=b, frame=single}
    \begin{lstlisting}[language=Python, caption=Example of style parameters for one artist.]
    if style == 'Tobu':
        lead_names = ['Forever', 'Stars', 'Blue']
        chord_names = ['Massive', 'Supersaws']
        bass_names = ['Home', 'Perfect']
        sub_names = ['SUBBASS']
        balance = {
            'lead': -9, 'chord': -15, 'bass': -6, 'sub': -9
        }
    \end{lstlisting}
    
    Then, for the lead part, we define a pattern core and use each of the lead synth to build a layer of the lead melody and add that to the pattern core, as shown in Listing 2. Note that the melody notes are symbolic representations parsed by utility functions available in the source code. We also do the same for chord layers, bass layers and sub-bass layers. For clarity, their code snippets are omitted but are open-sourced \href{https://github.com/Gariscat/loopy/blob/master/loopy/template.py}{\color{blue}{here}}.
    
    \begin{lstlisting}[language=Python, caption=Building the pattern for lead instruments.]
    ld_core = LoopyPatternCore(num_bars=8)
    for i, lead_name in enumerate(lead_names):
        generator = LoopyPreset(
            source_path=find_preset(
                preset_dir=f'Ultrasonic-LD-{lead_name}.wav'
            ),
            name=f'LEAD-{i}',
        )
        ld_core.add_notes(melody_notes, generator)
    \end{lstlisting}
    
    Before putting the pattern cores into the track, we also need to build the mixer channel for each pattern, or in other words, for each part (lead, chord, bass, sub-bass). A typical mixer channel contains effects like EQ, compression, sidechain automation, etc. Some might also include reverberation, delay and distortion. In Listing 3, we give an example of our default mixer channel. For consistency, we use the channel for lead synthesizers to demonstrate out setup. The waveform would sequentially go through a highpass filter with cutoff equal to 500 Hz, a volume balance, a sidechain effect and a reverberation. The sidechain effect an essential part of EDM songs and its details would be discussed in Appendix \ref{appendix:sidechain}.
    
    \begin{lstlisting}[language=Python, caption=Building the channel for lead instruments.]
    lead_channel = LoopyChannel(
        name='LEAD',
        effects=[
            LoopyHighpass(500),
            LoopyBalance(balance['lead']),
            LoopySidechain(
                attain=1/2,
                interp_order=2,
                mag=0.5
            ),
            LoopyReverb(wet_level=0.5),
        ]
    )
    \end{lstlisting}
    
    
    Finally, we put the pattern cores into the track and add the drum kit. As mentioned in section 4.1, the pattern cores are "skeletons" that do not include metadata, such as where the pattern is placed in the track and which mixer channel it belongs to when rendering the sound. The \code{add\_pattern} function of the \code{LoopyTrack} class creates an actual pattern with position and channel information and put it in the track. In Listing 4, the global position is the bar index and while the local position is the beat index. Here, the two $0$'s mean that the created pattern is placed at the very beginning of the track.
    
    \begin{lstlisting}[language=Python, caption=Putting the pattern (core) into the track and add the drum kit.]
    cores = (ld_core, ch_core, bs_core, sb_core)
    channels = (
        lead_channel, chord_channel, bass_channel, sub_channel
    )
        
    for core, channel in zip(cores, channels):
        track.add_pattern(
            pattern_type=core,
            global_pos=0,
            local_pos=0,
            channel=channel
        )
    
    add_kick(track=track, num_bars=8)
    add_clap(track=track, num_bars=8)
    add_hat(track=track, num_bars=8)
    \end{lstlisting}
    
    The tedious details above are wrapped up as a template function \code{prog\_house} with 2 required arguments \code{melody\_line} and \code{chord\_line}, returning \code{LoopyTrack} instance. The \code{melody\_line} and \code{chord\_line} are essentially 2 list of integers specifying the melody and the chord progression of a track, being extremely convenient to handle as symbolic representations. The audio of the track could be rendered using just 1 line of code \code{track.render()}. All information of the track, from metadata to mixer channels and pattern/sample positions, could be saved by simply calling \code{track.save()}.
\end{comment}
